Predicting Evoked Emotions in Conversations

Understanding and predicting the emotional trajectory in multi-party multi-turn conversations is of great significance. Such information can be used, for example, to generate empathetic response in human-machine interaction or to inform models of pre-emptive toxicity detection. In this work, we introduce the novel problem of Predicting Emotions in Conversations (PEC) for the next turn (n+1), given combinations of textual and/or emotion input up to turn n. We systematically approach the problem by modeling three dimensions inherently connected to evoked emotions in dialogues, including (i) sequence modeling, (ii) self-dependency modeling, and (iii) recency modeling. These modeling dimensions are then incorporated into two deep neural network architectures, a sequence model and a graph convolutional network model. The former is designed to capture the sequence of utterances in a dialogue, while the latter captures the sequence of utterances and the network formation of multi-party dialogues. We perform a comprehensive empirical evaluation of the various proposed models for addressing the PEC problem. The results indicate (i) the importance of the self-dependency and recency model dimensions for the prediction task, (ii) the quality of simpler sequence models in short dialogues, (iii) the importance of the graph neural models in improving the predictions in long dialogues.

==> 4-Method-old.tex <==
\section{Models}

%In order to derive the predictions we use a time series  Long Short Term Memory (LSTM) for both the emotion series prediction problem described in research question Q2 and the text series prediction problem described in research question Q3. The data classes are severely imbalanced as shown in Table \ref{table:2}, thus minority classes have all false negative predication's in favor of the majority class ``neutral". For this reason we used a number of techniques to handle the imbalanced data. Below we describe the specifics of handling the imbalanced data, training the prediction model and the tests we ran to allow for a more informed PEC model.

%In our methodology we differentiate between a series of utterance emotions and utterance sentences(text). The following two sections explain the methodology used to predict the next emotion given a sequence of emotions only and the methodology used to predict the next emotion given a sequence of text only.huihihigfguygigigigihiucccccchhyhhhhlljokokopkuhihiihjoicgjvjvjygbjnunnunnnknkknknkdevcev dev devmjojoiknijijnijijijinomojmkmomomomomokcttf     vcvvcfcdfdrdtrfgfgggggg cb  vbnnvujjjjbybjgmggggggggggggggggggkjnbnngbngn


We explore four variations  for the next emotion prediction NEP model: \\
\noindent
\textbf{Emotion Sequence}: The problem of next emotion prediction given a sequence of emotion transitions is similar to time series prediction. In this case, we only have the emotion labels $\mathcal{C}^{(u)}=\{ e_1^{(u)},e_2^{(u)},...,e_n^{(u)}\}$, $e \in \mathcal{E}$ which is one-hot encoded into a vector of size $|\mathcal{E}|$, with each dimension representing one of the emotion categories. Here a time series BiLSTM model with activation `ReLu' and a Dense layer with activation `softmax' is used to output the predicted label $e_{n+1}$. \\
\noindent
\textbf{Text Sequence}: We use the text utterances $\mathcal{C}=\{ t_1^{(u)},t_2^{(u)},...,t_n^{(u)}\}$ to predict $e_{n+1}$.
%The text sequences are first cleaned by removing the stopwords, removing punctuation and converting to lower case followed by lemmatization. Then, 
Following standard text pre-rpcoessing
each textual utterance is converted into a vector representation using the GloVe word embeddings \cite{pennington2014glove}. Then a Time Distributed layer followed by a Flatten layer are used before passing the input to a BiLSTM model.\\
\noindent
\textbf{Emotion + Text Sequence}: In this model, the emotion sequences and the text sequences, $\mathcal{C}=\{ \langle t_1, e_1 \rangle ^{(u)} , \langle t_2, e_2 \rangle ^{(u)} ,..., \langle t_n, e_n \rangle ^{(u)} \}$, are fed separately into two LSTMs, which are then concatenated for prediction. 

For each of the models we identify two common properties: (i) The length of the temporal window, how far the temporal window extends into the past upon which which estimation relies explicitly, and (ii) The nature of the user dependency, does the model rely on ly on the utterances of the sepaker being modeled (self dependency), or on both sides oft he conversation (dyadic dependency).

%\textbf{User dependency}: The final model incorporates two types of user information: self-dependency which only considers the information originating from the user $u$ for which $e_{n+1}^{(u)}$ is to be predicted. For instance, assuming $u=A$, the input is of the form 

%$\mathcal{C}=\{ \langle t_i^{(u=1)},e_i^{(u=1)}\rangle \}$.
%$\mathcal{C}=\{ \langle t_1,e_1\rangle ^{(A)}, ..., \langle t_n,e_n\rangle ^{(A)} \}$.
 
%\textcolor{blue}{please see how to best describe the following -- there are two types of user dependencies we explored: self-dependency, and ``other" / inter? dependency. Basically, for the target variable $e_{n+1}$, if it is user A's turn, then we consider all past data from only user A and call it self-dependency. and if we consider all data from the 'other' user B, then we call it ... OLB (other look back). can rename better if needed.}

\begin{comment}
This is a time series LSTM model which has a number of $time-steps=i$ based on the upper bound in each investigation. The time steps is the number of emotion look backs in the conversation used to predict the next emotion. 
\begin{enumerate}
    \item The input is a series of emotions each emotion is converted into a vector of 7 dimensions, each dimension represents one of the emotions. That is, a one hot shot encoding. 
    \item A  Bi-directional LSTM with activation `relu', that goes through each utterance emotion at a time.
    \item A Dense layer with activation `softmax' with an output of dimension  7 mapping to one of the classes as the predicted emotion for the next utterance.
\end{enumerate}

 We compile the model with loss categorical cross entropy,  also called Softmax Loss. It is a Softmax activation plus a Cross-Entropy loss. If we use this loss, we will train a LSTM to output a probability over all the  classes for one conversation history. It is used for multi-class classification. Below is the function:
 \begin{center}
   \textbf{$LOSS_{y'} (y) = - \sum_{i} y_{i}' \log (y_i)$  }
 \end{center}

We compile the model with Adam optimizer which is an adaptive learning rate optimization algorithm that’s been designed specifically for training deep neural networks. Adam performs a weight update given the following equation, where w is model weights, m and v are moving averages hyper-parameters, and eta (looks like n)is the step size:
 \begin{center}
\textbf{$w_{t+1} = w_{t} - \dfrac{\eta}{\sqrt{\hat{v}_t} + \epsilon} \hat{m}_t$}
  \end{center}
\end{comment}






%\begin{enumerate}  \item  Clean the text by removing stop words, changing text to lower case, removing punctuation and  removing bad characters. \item Lemmatize the text to transform the words to the actual root. \item Tokenize to construct a unique word dictionary and assign an integer to every word. \item Convert the sequences into a well-structured matrix so our learning model knows the number of feature dimensions. To do so, we define the max number of words in a sentence to be 20 and apply a post padding and post truncation. \end{enumerate}


%This is a time series LSTM model which has a number of $time-steps=i$ based on the upper bound in each investigation. The time steps is the number of text phrase look backs in the conversation used to predict the next emotion. Before we feed the text into the learning model we pre-process the data as shown in the following section. This helps the model select the appropriate features but also helps reduce the number of features as text classification problems have a high chance of over-fitting due to a high number of features.
 
 
%Once the text is ready to be fed into the learning model, we generate the embedding matrix. The sequences are then created using the glove 6B 300 dimension embeddings, which in turn are fed into the LSTM model one sentence at a time then one word at a time. 

\begin{comment}
\begin{enumerate}
    \item The input of our deep learning model is an Embedding layer. The embedding matrix is a matrix of row size equal to the number of unique words in the dataset  and has a column size of the embedding vector dimension, which is 300, that provides the word weight.
    \item The input is reconstructed as a series of 20 words for each sentence which translates to a 300 dimension embedding representation for each word multiplied by 20, which is the number of max words in a sentence. So each unit of time in our time series model takes a 6000 dimension for each sentence.  
    \item A Time Distributed and flatten layer that encapsulates the 6000 dimension sentence representation in each time step and forwards that to the LSTM. 
    \item A  Bi-directional LSTM Layer with activation 'relu' ,that walks through the sentences  each word at a time, that is 20 words with a 300 dimension. The output is 300 units. 
    \item A Dense layer with activation 'softmax' that takes 300 units and outputs 7, predicting  one of the classes as the emotion for the next utterance.
\end{enumerate}
 Similar to the emotion series model we compile this model with loss categorical cross entropy and an  Adam optimizer.
\end{comment}










%This is a multi-input time series LSTM model which has a number of $time-steps=i$ based on the upper bound in each investigation. The time steps is the number of text phrase look backs in the conversation used to predict the next emotion. This model concatenates the emotion series and text series model and joins at the dense layer which is the last layer in both the series making the predication by concatenating both input features. 

 
 
 





==> 8-Tables.tex <==
 

\begin{comment}
\begin{table*}[h]
\resizebox{\textwidth}{!}{%
\centering
 \begin{tabular}{||c|c| e|f |g |c|e|f |g |c| e|f |g |c| e|f |g ||} 
   \hline
 \multicolumn{17}{||c||}{Comparison of methods to counter imbalanced classes in the emotion series}\\ 
  \hline
    Upper-bound&\multicolumn{4}{c|}{$i=1$}&\multicolumn{4}{c|}{$i=2$} &  \multicolumn{4}{c|}{$i=3$} & \multicolumn{4}{c||}{$i=4$} \\ 
 \hline
  \hline
 Method &NoB & SW & CW & OVS  &NoB  & SW & CW & OVS &NoB  & SW & CW & OVS &NoB & SW & CW & OVS\\  
 \hline\hline
Neutral   &.92  &   .92 & .90 &.90  & .91 &   .92 & .89 &.89 & .91  &   .91 & .85 &.85 & .92  &   .91 & .84 &.85\\
 \hline
Anger  &0  &  0 &.14 & .14 &.56 &  .56 &.43 & .43 &.56  &  .54 &.41 & .28& 0  &  .49 &.37 & .36\\
 \hline
Disgust  &0  &  0& .03 &.03  &0  & .48 & .35 & .35 &.05& .43 & .31 & .35  & 0 & .41 & .29 & .29\\
 \hline
Fear    &0 &   0 & 0 & 0    &0 & .29 & .22 & .26 & 0 & .29 & .24 & .25 & 0  &   .34 & .28 & .21  \\
 \hline
Happiness   &.54   &  .54 & .54 & .54  &.49  &  .49 & .57 & .57 & .55   &  .55 & .56 & .56 & .54 &  .45 & .54 & .54\\
 \hline
Sadness   &0  &   0  & .07& .07  &0  &.28  & .22& .23& 0 &   .38  & .29 & .29 & 0 &   .32  & .2 & .16\\
 \hline

Surprise   &0   &   0 & 0& 0   &0  &   0 & .13& .14  & 0&  0 & .07 & .08 & 0  &   .01 & .06 & .07\\
 \hline
  \rowcolor{Gray2}
 macro avg   &.21 & .21 & .24 & .24 &.28  & .43 & .40 & .41& .30 & .44 & .39 & .38& .21  & .42 & .37 & .35 \\
 \hline
  \rowcolor{Gray1}
 loss  & .53& .55 & 1.83 & 1.82  &.523 & .5 & 1.54 & 1.52 & .491 &.5 & 1.53 & 1.56 & 0.548  & .49 & 1.5 & 1.44 \\
 \hline

\end{tabular}%
}
\caption{Accuracy of prediction on each emotion class in the Dailydialog dataset with look back $i=1$, $i=2$, $i=3$ and $i=4$, where NoB= No-Balancing, SW = Smoothen-Weights, CW = Count-Weights and OVS = OVer-Sampling. }
\label{table:primedatasets}
\end{table*}
    
\end{comment}



\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c| r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u | r| >{\color{red}}s |>{\color{blue}}t||}
 \hline
  \multicolumn{15}{|c|}{\textbf{Emotion series:} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
Upper-bound &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$} &  \multicolumn{3}{c|}{$i=$8}  \\ 
 \hline
 \hline
 Method & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB & 8LB & 4SLB & 4OLB\\  
 \hline\hline
Neutral   &   .91 & .91 &.91 &.89 &   .90 & .89 &.89  & .89 &.90 &.90  & .90 &   .89 & .89 &.89\\
 \hline
Anger &  .49 &.52 & .50 &0 &  .46 &.44 & .44 &.44 &0 &0 &0  &  .46 &.44 & 0 \\
 \hline
Disgust  & .41 & .40 & .45& 0 & .26 & .27 & .31  & .42 &0 &0 &0 & .22 & .20 & 0\\
 \hline
Fear   &   .34 & .47 & .49 &0 &   .37 & .18 & .24  & .43&0 &0 &0   &   .00 & .20 & 0\\
 \hline
Happiness    &  .45 & .45 & .54 &.53&  .36 & .34 & .33  & .46  &.56 &.56 &.56    &  .52 & .36 & .53 \\
 \hline
Sadness   &   .32  & .32 & .33&0    &   .27  & .31 & .31 & .41 &0 &0 &0  &   .30  & .34 & 0\\
 \hline
Surprise    &   .01& 0 & 0 &0    &   .02 & .06 & 0  & 0 &0 &0 &0   &   .03 & .03 & 0\\
 \hline
 \rowcolor{Red}
 macro avg& .42 & .44 & .45 &.20& .38 & .36 & .36  & .44&.21 & .21&.21 & .35 & .35 & .20 \\
 \hline
 \rowcolor{Blue}
  loss & 0.55 & 0.55 & 0.55 &0.6 & 0.57 & 0.57 & 0.57 & .59&.578 &.584 &.589 & 0.57 & 0.57 & 0.59\\
 \hline
\end{tabular}%
}
\caption{Accuracy of prediction on each emotion class in the text series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB= 4-look-backs, 3LB= 3-look-backs, 2LB=  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB= 3-self-dependency-look-back, 2SLB= 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB= 3-inter-dependency-look-back, 2OLB= 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back.  }
\label{table:emotionlookbacks}
\end{table*}







\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c|r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u||} 
 \hline
  \multicolumn{12}{|c|}{\textbf{Text series:} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
  Upper-bound   &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$}  \\ 
 \hline
 \hline
 Method  & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB\\
 \hline\hline
Neutral  & .90 &.90 & .90  & .89   & .89  & .88 &.87  & .87 &.88 &.88  & .87\\
 \hline
Anger & .30 &.23 & .27 & .32& .33 &.40 & .30 &.35 &.24 &.24&.32   \\
 \hline
Disgust &.47  &.27 & .29 & .21 & .22 & 0 & .40  & .15 &0 &0 &.17  \\
 \hline
Fear  & .42 & .27& .12 & 0 &  .67 & .67 & .25  & .40&.57 &.46&.25  \\
 \hline
Happiness &.51  & .45 & .35 & .26 &  .48 & .38 & .34  & .30  &.34 &.38 &.35 \\
 \hline
Sadness  & .11 & .13& .23 & .17 &  .28 & .15 & .33 & .18 &.36 &13 &.30 \\
 \hline
Surprise  & .16 & .26& .22 & .25 & .30   & .36 & .18  & .23 &.21 &33 &.10\\
 \hline
 \rowcolor{Red}
 macro avg& .41 &.36 & .34 & .30 &.45 & .41 & .38  & .35&.37 & .35&.34 \\
 \hline
 \rowcolor{Blue}
  loss & .722 & .71& .788 & .801& .904 & 1.088 & 1.097 & 1.023& 1.189 & 1.086 &1.008   \\
 \hline
\end{tabular}
}    
\caption{Accuracy of prediction on each emotion class in the emotion series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB = 4-look-backs, 3LB = 3-look-backs, 2LB =  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB = 3-self-dependency-look-back, 2SLB = 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB = 3-inter-dependency-look-back, 2OLB = 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back. Last, with look backs on upper-bound $i=8$,  and selected features 8LB = 8-look-back, 4SLB = 4-self-dependency-look-back and 4OLB = 4-inter-dependency-look-back. }
\label{table:textlookbacks}
\end{table*}





\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c|r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u||} 
 \hline
  \multicolumn{12}{|c|}{\textbf{Emotion and Text series combined :} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
    Upper-bound &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$}  \\ 
 \hline
 \hline
 Method  & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB\\
 \hline\hline
Neutral  & .91  & .91& .91 & .90  & .89  &.88 &  .87&.87 & .86 & .87  & .89 \\
 \hline
Anger & .37& .46 & .38&.22 & .40 & .39& .48 &.43 & .49 &  .39 & .29  \\
 \hline
Disgust & .23  &.16 & .18 & .19 & .06 & .08& .08 &0 & .08 &  0 & 0  \\
 \hline
Fear  & .29 &.39 & .38 & .23 &  .29  & .33& .27 & .34& .25 & .33  & .17  \\
 \hline
Happiness&.55  &.54 & .51 &.46  & .57 &.54 & .48 & .40& .50 &  .52 & .52 \\
 \hline
Sadness  & .24 &.17 & .27 & .14 & .16   &.23 & .28 &.18 & .23 & .16  & .16  \\
 \hline
Surprise  & .23  &.23 & .21 & .18 &  .21  & .17& .25 & .15&  .25&  .18 & .22  \\
 \hline
 \rowcolor{Red}
 macro avg&.40  & .41 & .41 & .33 & .37 & .38&  .39&.34 & .38 &  .35 & .32 \\
 \hline
 \rowcolor{Blue}
  loss & .853 & .865& .917 & .882 &1.021 &.931 & .958 &.912 & 1.003 & .981  & .892   \\
 \hline
\end{tabular}
}    
\caption{Accuracy of prediction on each emotion class in the emotion series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB= 4-look-backs, 3LB= 3-look-backs, 2LB=  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB= 3-self-dependency-look-back, 2SLB = 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB = 3-inter-dependency-look-back, 2OLB = 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back. Last, with look backs on upper-bound $i=8$,  and selected features 8LB = 8-look-back, 4SLB= 4-self-dependency-look-back and 4OLB = 4-inter-dependency-look-back. }
\label{table:textemotion}
\end{table*}



==> full-tables.tex <==


\subsection{Results}

To solve our research question, we restructure our data with different values of our conversation phrase upper bound $i$. So, if $i=1$ we restructure the data to take all pair turns in every conversation, where we predict the next emotion given the previous emotion. If $i=2$ we restructure the data to include three turns where we predict the next emotion given the previous two, and so on for every  upper-bound $i$ under investigation. This results in an different emotion label distribution. In our investigations we considered the upper-bounds $i$ shown in Table \ref{table:2}. After this restructuring we have a number of prime data-sets that are used to train our emotion prediction model. 
\subsection{Handling imbalanced  data }
We first define three different variants of our prediction model that handle the imbalanced classes. The SW model uses smoothen weights, the CW uses count weights and the OVS uses over-sampling as described in our methodology section.  We then use these variants to predict the next emotion  given  a number of upper-bound $i=1,2,3$ and $4$. The results of these predictions are shown in table \ref{table:primedatasets}. The results show that SW had the best performance, thus was chosen to be used for the continuity of our tests. 
\begin{table*}[h]
\resizebox{\textwidth}{!}{%
\centering
 \begin{tabular}{||c|c| e|f |g |c|e|f |g |c| e|f |g |c| e|f |g ||} 
   \hline
 \multicolumn{17}{||c||}{Comparison of methods to counter imbalanced classes in the emotion series}\\ 
  \hline
    Upper-bound&\multicolumn{4}{c|}{$i=1$}&\multicolumn{4}{c|}{$i=2$} &  \multicolumn{4}{c|}{$i=3$} & \multicolumn{4}{c||}{$i=4$} \\ 
 \hline
  \hline
 Method &NoB & SW & CW & OVS  &NoB  & SW & CW & OVS &NoB  & SW & CW & OVS &NoB & SW & CW & OVS\\  
 \hline\hline
Neutral   &.92  &   .92 & .90 &.90  & .91 &   .92 & .89 &.89 & .91  &   .91 & .85 &.85 & .92  &   .91 & .84 &.85\\
 \hline
Anger  &0  &  0 &.14 & .14 &.56 &  .56 &.43 & .43 &.56  &  .54 &.41 & .28& 0  &  .49 &.37 & .36\\
 \hline
Disgust  &0  &  0& .03 &.03  &0  & .48 & .35 & .35 &.05& .43 & .31 & .35  & 0 & .41 & .29 & .29\\
 \hline
Fear    &0 &   0 & 0 & 0    &0 & .29 & .22 & .26 & 0 & .29 & .24 & .25 & 0  &   .34 & .28 & .21  \\
 \hline
Happiness   &.54   &  .54 & .54 & .54  &.49  &  .49 & .57 & .57 & .55   &  .55 & .56 & .56 & .54 &  .45 & .54 & .54\\
 \hline
Sadness   &0  &   0  & .07& .07  &0  &.28  & .22& .23& 0 &   .38  & .29 & .29 & 0 &   .32  & .2 & .16\\
 \hline

Surprise   &0   &   0 & 0& 0   &0  &   0 & .13& .14  & 0&  0 & .07 & .08 & 0  &   .01 & .06 & .07\\
 \hline
  \rowcolor{Gray2}
 macro avg   &.21 & .21 & .24 & .24 &.28  & .43 & .40 & .41& .30 & .44 & .39 & .38& .21  & .42 & .37 & .35 \\
 \hline
  \rowcolor{Gray1}
 loss  & .53& .55 & 1.83 & 1.82  &.523 & .5 & 1.54 & 1.52 & .491 &.5 & 1.53 & 1.56 & 0.548  & .49 & 1.5 & 1.44 \\
 \hline

\end{tabular}%
}
\caption{Accuracy of prediction on each emotion class in the Dailydialog dataset with look back $i=1$, $i=2$, $i=3$ and $i=4$, where NoB= No-Balancing, SW = Smoothen-Weights, CW = Count-Weights and OVS = OVer-Sampling. }
\label{table:primedatasets}
\end{table*}
\subsection{Emotion series}
In this section we analyze the results of tests on the emotion series in a conversation. This work analyzes look backs that take all the emotional history of  both speakers in a conversation to predict the next emotion, these are called general look backs. This work  also analyses speaker specific emotional history in the conversation for the same purpose. 
\subsubsection{General look backs:}
Table \ref{table:primedatasets} shows that best results are achieved with a two step look back shown in the $i=2$ part of the table, and the worst results are with a one step look back shown in the  $i=2$ part of the table. These results are confirmed in Table \ref{table:emotionlookbacks} in the $i=4$ upper bound part of the table, here we use this prime dataset and perform looks backs up to the upper-bound $i=4$. The results in Table \ref{table:emotionlookbacks} were generated to compare the variations of look backs on one prime reconstruction of the original dataset. That is to use the same training and testing set on all these look backs for a more sound comparison.  As shown a two step look-back gives best results and the accuracy suffers with more looks. The worst result was with a 1 step look back.

\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c| r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u | r| >{\color{red}}s |>{\color{blue}}t||}
 \hline
  \multicolumn{15}{|c|}{\textbf{Emotion series:} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
Upper-bound &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$} &  \multicolumn{3}{c|}{$i=$8}  \\ 
 \hline
 \hline
 Method & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB & 8LB & 4SLB & 4OLB\\  
 \hline\hline
Neutral   &   .91 & .91 &.91 &.89 &   .90 & .89 &.89  & .89 &.90 &.90  & .90 &   .89 & .89 &.89\\
 \hline
Anger &  .49 &.52 & .50 &0 &  .46 &.44 & .44 &.44 &0 &0 &0  &  .46 &.44 & 0 \\
 \hline
Disgust  & .41 & .40 & .45& 0 & .26 & .27 & .31  & .42 &0 &0 &0 & .22 & .20 & 0\\
 \hline
Fear   &   .34 & .47 & .49 &0 &   .37 & .18 & .24  & .43&0 &0 &0   &   .00 & .20 & 0\\
 \hline
Happiness    &  .45 & .45 & .54 &.53&  .36 & .34 & .33  & .46  &.56 &.56 &.56    &  .52 & .36 & .53 \\
 \hline
Sadness   &   .32  & .32 & .33&0    &   .27  & .31 & .31 & .41 &0 &0 &0  &   .30  & .34 & 0\\
 \hline
Surprise    &   .01& 0 & 0 &0    &   .02 & .06 & 0  & 0 &0 &0 &0   &   .03 & .03 & 0\\
 \hline
 \rowcolor{Red}
 macro avg& .42 & .44 & .45 &.20& .38 & .36 & .36  & .44&.21 & .21&.21 & .35 & .35 & .20 \\
 \hline
 \rowcolor{Blue}
  loss & 0.55 & 0.55 & 0.55 &0.6 & 0.57 & 0.57 & 0.57 & .59&.578 &.584 &.589 & 0.57 & 0.57 & 0.59\\
 \hline
\end{tabular}%
}
\caption{Accuracy of prediction on each emotion class in the text series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB= 4-look-backs, 3LB= 3-look-backs, 2LB=  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB= 3-self-dependency-look-back, 2SLB= 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB= 3-inter-dependency-look-back, 2OLB= 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back.  }
\label{table:emotionlookbacks}

\end{table*}

\subsubsection{Speaker dependent look backs:}
Table \ref{table:emotionlookbacks} shows the inter-dependency and self-dependency on the speaker of the predicated emotion using the prime data-set with upper bound $i=6$ and upper bound $i=8$. These upper-bounds where chosen to display the results as they provide an even distribution of turn utterances between speaker A ad B. So, for upper-bound $i=6$ there are 3 turns for speaker A and B , and for  upper-bound $i=8$ there are 4 turns for speaker A and B. The results in the upper-bound $i=8$ part of the table show that using the emotion history of all the 8 turns gives similar performance to using the emotion history of the 4 turns of the same speaker of the predicted emotion. The results in the upper-bound $i=8$ part of the table also show that using the 4 turn of the speaker other that the speaker of the predicated emotion gives considerably worse results.  These results suggest speaker self-dependency when predicting emotions. To further confirm these results, in the upper-bound $i=6$ part of the table, it shows that all look backs belonging to the same speaker give a higher performance when compared to their counter parts for the other speaker. When comparing the speaker of the predicated emotions own look backs, it can be seen that a 1 look back for the same speaker shows best performance. In fact, the 1 look back of the same speaker gives the highest performance among all performances.

\subsection{Text series}
In this section we analyze the results of tests on the text series in a conversation. This work analyzes look backs that take all the textual history of  both speakers in a conversation to predict the next emotion, these are called general look backs. This work  also analyses speaker specific textual history in the conversation for the same purpose.  

\subsubsection{General look backs:}
 Table \ref{table:textlookbacks}  shows that more textual history  results in better performance. so the more the look-backs the better the result. This result is confirmed in both the upper-bound $i=6$ and $i=4$ part of the table, showing consistent results on both prime data-sets.  
\begin{table*}[h]

\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c|r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u||} 
 \hline
  \multicolumn{12}{|c|}{\textbf{Text series:} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
  Upper-bound   &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$}  \\ 
 \hline
 \hline
 Method  & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB\\
 \hline\hline
Neutral  & .90 &.90 & .90  & .89   & .89  & .88 &.87  & .87 &.88 &.88  & .87\\
 \hline
Anger & .30 &.23 & .27 & .32& .33 &.40 & .30 &.35 &.24 &.24&.32   \\
 \hline
Disgust &.47  &.27 & .29 & .21 & .22 & 0 & .40  & .15 &0 &0 &.17  \\
 \hline
Fear  & .42 & .27& .12 & 0 &  .67 & .67 & .25  & .40&.57 &.46&.25  \\
 \hline
Happiness &.51  & .45 & .35 & .26 &  .48 & .38 & .34  & .30  &.34 &.38 &.35 \\
 \hline
Sadness  & .11 & .13& .23 & .17 &  .28 & .15 & .33 & .18 &.36 &13 &.30 \\
 \hline
Surprise  & .16 & .26& .22 & .25 & .30   & .36 & .18  & .23 &.21 &33 &.10\\
 \hline
 \rowcolor{Red}
 macro avg& .41 &.36 & .34 & .30 &.45 & .41 & .38  & .35&.37 & .35&.34 \\
 \hline
 \rowcolor{Blue}
  loss & .722 & .71& .788 & .801& .904 & 1.088 & 1.097 & 1.023& 1.189 & 1.086 &1.008   \\
 \hline
\end{tabular}
}    
\caption{Accuracy of prediction on each emotion class in the emotion series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB = 4-look-backs, 3LB = 3-look-backs, 2LB =  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB = 3-self-dependency-look-back, 2SLB = 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB = 3-inter-dependency-look-back, 2OLB = 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back. Last, with look backs on upper-bound $i=8$,  and selected features 8LB = 8-look-back, 4SLB = 4-self-dependency-look-back and 4OLB = 4-inter-dependency-look-back. }
\label{table:textlookbacks}

\end{table*}


\subsubsection{Speaker dependent look backs:}
Table \ref{table:textlookbacks} shows that when considering the textual history of the speaker whom we are predicting the  next emotion, the results are better in comparison to considering the textual history of the other speaker. However, considering the overall textual history gives better results overall. This suggests that part of the truth is self-dependent on the same speaker and the other part is inter-dependent on the other speaker. How much of the truth lies in each part is a question yet to be discovered.

\begin{table*}[h]

\centering
\resizebox{\textwidth}{!}{%
 \begin{tabular}{||c|r|s |t |u| r|>{\color{red}}s |>{\color{red}}t |>{\color{red}}u|>{\color{blue}}s |>{\color{blue}}t |>{\color{blue}}u||} 
 \hline
  \multicolumn{12}{|c|}{\textbf{Emotion and Text series combined :} Comparison of general, self-dependency and inter-dependency look backs }\\ 
 \hline
    Upper-bound &\multicolumn{4}{c|}{$i=4$}&\multicolumn{7}{c|}{$i=6$}  \\ 
 \hline
 \hline
 Method  & 4LB & 3LB & 2LB & 1LB& 6LB & 3SLB & 2SLB & 1SLB &3OLB & 2OLB & 1OLB\\
 \hline\hline
Neutral  & .91  & .91& .91 & .90  & .89  & &  &.91 &  &   &  \\
 \hline
Anger & .37& .46 & .38&.22 & .40 & &  &.38 &  &   &    \\
 \hline
Disgust & .23  &.16 & .18 & .19 & .06 &&  &0 &  &   &   \\
 \hline
Fear  & .29 &.39 & .38 & .23 &  .29  & &  & .31&  &   &   \\
 \hline
Happiness&.55  &.54 & .51 &.46  & .57 & &  & .34&  &   &   \\
 \hline
Sadness  & .24 &.17 & .27 & .14 & .16   & &  &.14 &  &   &   \\
 \hline
Surprise  & .23  &.23 & .21 & .18 &  .21  & & .11 & &  &   &  \\
 \hline
 \rowcolor{Red}
 macro avg&.40  & .41 & .41 & .33 & .37 & &  &.31 &  &   &  \\
 \hline
 \rowcolor{Blue}
  loss & .853 & .865& .917 & .882 &1.021 & &  &.912 &  &   &    \\
 \hline
\end{tabular}
}    
\caption{Accuracy of prediction on each emotion class in the emotion series using SW: Starting  with look backs on upper-bound $i=4$, and selected features 4LB= 4-look-backs, 3LB= 3-look-backs, 2LB=  2-look-backs and 1LB= 1-look-back. Next, with look backs on upper-bound $i=6$, and selected features 6LB= 6-look-back, 3SLB= 3-self-dependency-look-back, 2SLB = 2-self-dependency-look-back and 1SLB = 1-self-dependency-look-back, 3OLB = 3-inter-dependency-look-back, 2OLB = 2-inter-dependency-look-back and 1OLB = 1-inter-dependency-look-back. Last, with look backs on upper-bound $i=8$,  and selected features 8LB = 8-look-back, 4SLB= 4-self-dependency-look-back and 4OLB = 4-inter-dependency-look-back. }
\label{table:textemotion}

\end{table*}
\subsection{Emotion and text series combined}
\subsubsection{General look backs:}
\subsubsection{Speaker dependent look backs:}


